Microcirculatory blood flow with aberrant levels of red blood cell aggregation

Recent clinical results indicate that aberrant erythrocyte aggregation in hematological disorders is accompanied by endothelial damage and glycocalyx disruption, but the underlying biophysical mechanisms remain unclear. This study uses direct computational modeling to explore how red blood cell (RBC) aggregation impacts shear stress in small blood vessels, highlighting the increased risk of vascular damage. RBC aggregation creates a heterogeneous distribution, leading to variations in the cell-free layer thickness and fluctuating wall shear stress, especially near vessel walls. This effect aligns with experimental findings on endothelial disruption linked to RBC clustering near the wall, potentially reducing the protective glycocalyx layer. The power spectral density analysis of wall shear stress fluctuations reveals that, with RBC aggregation, there is a distinct peak near frequency f = 0.04, indicating increased fluctuations due to aggregated RBC clusters traveling close to the vessel wall. The presence of aberrant cells in blood disorders, modeled here by sickle cells, further amplifies these effects, as aggregation-enhanced margination drives sickle cells closer to vessel walls, exacerbating shear stress fluctuations and increasing the likelihood of vascular injury and inflammation. Simulations show that curved vascular geometry, with curvature accentuating RBC clustering near vessel walls, intensifies aggregation-induced wall shear stress fluctuations and increases the risk of vascular damage, particularly in sickle cell disease where sickle cells marginate closer to the wall.

==> XCaggregationreview.tex <==
The advances in experiments contribute significantly to the understanding of blood cell aggregation dynamics \cite{faes2019red, bishop2002effect, claveria2021vitro, ong2010effect, brust2014plasma, flormann2017buckling, druzak2023multiplatform, nader2020red}. Bishop et al. \cite{bishop2002effect} investigated RBC variability in vivo, highlighting the impact of aggregation on velocity and shear rate. Claveria et al. \cite{claveria2021vitro} explored segregation of RBCs in sickle cell anemia, finding aggregation inhibition affects cell distribution, potentially influencing vascular adhesion. Ong et al. \cite{ong2010effect} observed enhanced cell-free layer formation in arterioles induced by fibrinogen-driven aggregation. Brust et al. \cite{brust2014plasma} revealed persistent aggregation in microcapillaries, impacting blood perfusion. Flormann et al. \cite{flormann2017buckling} analyzed diverse rouleaux morphologies and their quantitative recovery through simulations. Furthermore, studies on critically ill COVID-19 adults \cite{druzak2023multiplatform} and sickle cell disease \cite{nader2020red} highlight unique aggregation mechanisms and their implications in disease progression. These experiments collectively deepen our understanding of aggregation phenomena and their clinical significance.


Models of RBC aggregation are evolving to better understand this complex phenomenon. Neu and Meiselam \cite{neu2002depletion} introduced a method that calculates interaction energy between RBCs in polymer solutions, considering electrostatic repulsion and osmotic attractive forces. Liu et al. \cite{liu2004coupling, liu2006rheology} proposed a 3D model that incorporates depletion-mediated aggregation, revealing insights into shear rate-dependent viscosity, cell rigidity impact, and the Fahraeus-Lindqvist effect. Xu et al. \cite{xu2013large, xu2017investigation} investigated deformable RBC aggregation's effects on blood flow in the circulatory system in large-scale simulation. Fedosov et al. \cite{fedosov2011predicting} utilized coarse-grained molecular dynamics to predict blood viscosity dependence on shear rate and hematocrit, revealing reversible rouleaux structures and linking yield stress to cell aggregation, thus supporting experimental findings. 

The blood cell aggregation model, explored through various simulations and computational studies \cite{baskurt2011red, wang2009numerical, zhang2008red, bagchi2005computational, abbasi2021erythrocyte, zhang2009effects, fenech2009particle, lee2021numerical}, elucidate the formation of aggregated structures by blood cells and their impact on suspension properties and the cell-free layer. Zhang et al. \cite{zhang2008red} utilized an immersed boundary lattice Boltzmann algorithm to illustrate RBC behavior in shear flows, observing rouleau-like structures influenced by interaction strength. Bagchi et al. \cite{bagchi2005computational} simulated RBC aggregation, noting stable aggregate formation affected by cytoplasmic viscosity and membrane rigidity. Abbasi et al. \cite{abbasi2021erythrocyte} studied doublet dynamics under shear flow, showcasing stable doublet formation and its impact on viscosity. Zhang et al. \cite{zhang2009effects} reproduced microscopic blood flow features, including the cell-free layer and changes in viscosity. Fenech et al. \cite{fenech2009particle} explored the relationship between RBC interactions and rheological behavior, emphasizing the impact of aggregation force and shear rate on aggregate size. Lee et al. \cite{lee2021numerical} simulated RBC motion under pulsatile flow, revealing the role of shear rate distribution in aggregate formation. These studies collectively offer valuable insights into microscopic blood flows and their implications in various microcirculation scenarios.

Aggregation between cells significantly influences the cell-free layer (CFL). Ong et al. \cite{ong2011temporal} proposed increased arteriole CFL width variations due to aggregation. Aggregation notably augments layer width variations, improving NO bioavailability and sGC activation, potentially enhancing vascular tone. Furthermore, aggregation diminishes asymmetry in downstream vessel CFL widths, with a greater tendency for CFL formation in smaller downstream vessels under aggregating conditions \cite{ong2013effect}. Inducing aggregation in reduced flow conditions increases both the mean and standard deviation of layer width, especially pronounced in smaller arterioles \cite{ong2011cell}. Soutan et al. \cite{soutani1995quantitative}, examining erythrocyte aggregation's impact on microvessel dynamics, found that increased Dx-70 concentrations led to elevated erythrocyte suspension viscosity and CFL thickness, increasing flow resistance and causing uneven erythrocyte flow in microvessels.

Aggregation in various blood disorders, including diabetes, hyperviscosity syndrome, sickle cell diseases, malaria infection, and COVID-19, has been extensively studied, shedding light on their pathophysiology \cite{li2017biomechanics, nader2019blood, connes2014haemolysis, ballas2004sickle, kato2018sickle}. Deng et al. \cite{deng2020quantifying} investigated fibrinogen-dependent aggregation dynamics in type 2 diabetes mellitus (T2DM) red blood cells (RBCs), emphasizing the significance of aggregation dynamics in microvascular complications. Lei et al. \cite{lei2013probing} explored vasoocclusion crisis in sickle cell anemia using a multiscale model, revealing heterogeneous behavior among sickle RBC groups. Javadi et al. \cite{javadi2021silico} studied hyperviscosity syndrome, showing that factors such as plasma proteins, cell properties, and interactions influence blood viscosity. These studies collectively deepen our understanding of the pathophysiology of various blood disorders.

Moreover, Tripette et al. \cite{tripette2009red} highlighted the impact of red blood cell aggregation on microcirculatory blood flow dynamics in sickle cell disease, indicating challenges for single-cell passage through narrow capillaries. Ye et al. \cite{ye2014dissipative} simulated the deformation and aggregation of mixed healthy and malaria-infected RBCs, revealing altered dynamics with parasitic development. Dorken et al. \cite{dorken2023circulating} investigated circulating cellular clusters in COVID-19-induced immunothrombotic states, uncovering correlations with thrombotic complications and providing insights into microcirculatory obstruction. Alapan et al. \cite{alapan2016sickle} developed a microfluidic biochip for sickle cell disease, enabling quantitative assessment of RBC adhesion to endothelium-associated proteins, with potential applications in baseline assessments and therapeutic interventions. These studies collectively offer valuable insights into blood disorder pathophysiology and provide avenues for improved management strategies.

Cell aggregation in complex vascular geometries has also been studied, shedding light on its impact on blood flow dynamics \cite{li2020predictive, yazdani2017general, zheng2020three}. For instance, Xiao et al. \cite{xiao2020effects, xiao2016simulation} simulated microvascular stenosis fluid mechanics using dissipative particle dynamics to assess the impact of red blood cell (RBC) aggregation. Results revealed RBC accumulation upstream, leading to reduced flow velocity and increased blood flow resistance, potentially contributing to microthrombus formation. Chesnutt et al. \cite{chesnutt2009effect} explored plasma skimming in bifurcating microvascular vessels, showing significant plasma skimming in low-flow daughter branches with increased fractional particle flux at higher hematocrit. Bishop et al. \cite{bishop2001effects} found hindered formation of a cell-free marginal layer in the venular network due to time-dependent axial migration and frequent branching. Additionally, studies using microchannels with T-junctions \cite{sherwood2012effect} and T-type bifurcating microchannels \cite{kaliviotis2018local} demonstrated alterations in velocity profiles, CFL width, and local viscosity due to RBC aggregation. Sherwood et al. (2014) noted significant correlations between velocity and hematocrit profiles in microvascular channels, with asymmetry observed in plasma skimming at bifurcation points. These studies collectively deepen our understanding of the intricate dynamics of blood flow in complex vascular networks influenced by cell aggregation.

